The sandpile identity element on an ellipse

We consider certain elliptical subsets of the square lattice. The recurrent representative of the identity element of the sandpile group on this graph consists predominantly of a biperiodic pattern, along with some noise. We show that as the lattice spacing tends to 0, the fraction of the area taken up by the pattern in the identity element tends to 1.

==> DCDS_Identity_Elements_Sources.tex <==
\begin{thebibliography}{99}
% Example of an article in Academic Press or a book:
\bibitem{corry2018divisors}
    \newblock S. Corry and D. Perkinson,
    \newblock  Divisors and sandpiles,
    \newblock American Mathematical Soc., (2018), 33--75.

% Example of multiple authors:
\bibitem{fey2010growth}
    \newblock A. Fey, L. Levine and Y. Peres, % Use `and' connect the last two authors
    \newblock Growth rates and explosions in sandpiles,
    \newblock \emph{J. Stat. Phys.}, \textbf{138} (2010), 1-3.

% Example of a preprint article with 7 digits archive number:
\bibitem{jarai2014sandpile}
\newblock A.A. J{\'a}arai,
\newblock Sandpile models
\newblock preprint, \arXiv{math/1401.0354}.

% Example of multiple authors:
\bibitem{levine2016apollonian}
    \newblock L. Levine, W. Pegden and C.K. Smart, % Use `and' connect the last two authors
    \newblock Apollonian structure in the abelian sandpile,
    \newblock \emph{Geometric and functional analysis}, \textbf{26} (2016), 306-336.

% Example of multiple authors:
\bibitem{levine2017apollonian}
    \newblock L. Levine, W. Pegden and C.K. Smart, % Use `and' connect the last two authors
    \newblock Apollonian structure of integer superharmonic matrices,
    \newblock \emph{Annals of Mathematics}, (2017), 1-67.

\bibitem{pegden2020stability}
    \newblock W. Pegden and C.K. Smart, % Use `and' connect the last two authors
    \newblock Stability of patterns in the abelian sandpile,
    \newblock \emph{Annales Henri Poincar{\'e}}, (2020), 1-17.



\bibitem{stefani2016monotonicity}
\newblock G. Stefani,
\newblock On the monotonicity of perimeter of convex bodies
\newblock preprint, \arXiv{math/1612.00295}.



\end{thebibliography}
